Automatic Generation of Probabilistic Programming from Time Series Data

Probabilistic programming languages represent complex data with intermingled models in a few lines of code. Efficient inference algorithms in probabilistic programming languages make possible to build unified frameworks to compute interesting probabilities of various large, real-world problems. When the structure of model is given, constructing a probabilistic program is rather straightforward. Thus, main focus have been to learn the best model parameters and compute marginal probabilities. In this paper, we provide a new perspective to build expressive probabilistic program from continue time series data when the structure of model is not given. The intuition behind of our method is to find a descriptive covariance structure of time series data in nonparametric Gaussian process regression. We report that such descriptive covariance structure efficiently derives a probabilistic programming description accurately.

==> tikz_flows.tex <==
\newsavebox\mybox

\begin{lrbox}{\mybox}
\begin{tikzpicture}[transform canvas={scale=0.6}]

  \node[obs]                               	(y) {$y_i$};
  \node[latent, left=0.5cm of y] 				(fi) {$f_i$};
  \node[latent, left= 0.5cm of fi]  			(f) {$f$};
  \node[const, left=0.5cm of f]            	(gp) {$\mathcal{GP}$};
  \node[latent, left=0.7cm of gp]				(s) {$\sigma_j$};
  \node[const, below=0.5cm of gp]				(kj) {$k_{d_j}(x,x')$};
  \node[const, above=0.6cm of gp]				(ks) {$k_S(x,x')$};
  \node[const, left=0.5cm of ks]				(mu) {$\mu(x)$};
  \node[const, above=0.6cm of mu]				(zero) {$0$};
  \node[latent, right=0.4cm of zero]				(k_s) {$k_S$};
  \node[latent, right =1.6cm of zero]				(theta) {$\theta$};
   \node[const, above=0.5cm of k_s]				(g) {$G$};

%   \node[const, above= of gp, xshift=1.2cm]	(mu) {$\mu(x)$};

  \edge {fi} {y} ;
  \edge {f} {fi} ;
  \edge {gp} {f} ;
  \edge {kj} {gp};
  \edge {ks} {gp};
  \edge {mu} {gp};
  \edge {zero} {mu};
  \edge {g}{k_s};
  \edge {k_s}{ks};
  \edge {theta}{ks};

%   \edge {mu} {gp};
  \edge {s} {gp};

  % Plates
  \plate {fiyi} {(y) (fi)} {$i \in 1 ... N$};
  \plate {M} {(fiyi) (f) (gp) (kj) (s)} {$j \in 1 ... M$}


\end{tikzpicture}
\end{lrbox}

\begin{tikzpicture}[>=stealth,
    node distance=5cm,
    database/.style={
      cylinder,
      shape border rotate=90,
      aspect=0.25,
      draw
    }]
\begin{scope}[local bounding box=scope1]
\node[inner sep=0pt] (adjust) at (0,0)
    {\includegraphics[width=.20\textwidth]{./figure/adjust-close.png}};
\node[below right] at (adjust.south west) {\textbf{Multiple sequences}};
\draw[thick] ($(adjust.north west)+(-0.3,0.6)$) rectangle ($(adjust.south east) + (0.3,-0.6)$);
\end{scope}
\node[inner sep=0pt] (adjust) at (0,0)
    {\includegraphics[width=.20\textwidth]{./figure/adjust-close.png}};
\node[below right] at (adjust.south west) {\textbf{Multiple sequences}};

\node[inner sep=0pt, right=2cm of adjust] (gp){
\includegraphics[width=.20\textwidth]{./figure/model.pdf}
};
\node[below right] at (gp.south west) {\textbf{ABCD framework}};
\draw[thick] ($(gp.north west)+(-0.3,0.6)$) rectangle ($(gp.south east) + (0.3,-0.6)$);

\node[inner sep=0pt, above right=0.5cm and 1.5cm of gp] (c)
    {\includegraphics[width=.12\textwidth]{./figure/c.png}};

\node[inner sep=0pt, right=1cm of c] (se)
    {\includegraphics[width=.12\textwidth]{./figure/se.png}};

\node[inner sep=0pt, below= 0.5cm of c] (cp)
	{\includegraphics[width=.12\textwidth]{./figure/cp.png}};

\node[inner sep=0pt, below= 0.5cm of se] (mix)
	{\includegraphics[width=.12\textwidth]{./figure/mix.png}};

\node[inner sep=0pt, below= 1cm of adjust] (ind)
	{\includegraphics[width=.2\textwidth]{./figure/ind.png}};
\node[below right] at (ind.south west) {\textbf{Query}};

\node[database, right =1.2cm of ind] (db){Probabilistic programming};
\node[below right] at (db.south west) {\textbf{Stored \texttt{Stan}}  \textbf{codes}};

\node[inner sep=0pt, right= 2cm of db] (report)
	{\includegraphics[width=.15\textwidth]{./figure/report.png}};
\node[below right] at (report.south west) {\textbf{Report}};

\end{tikzpicture}


==> tikz_share_structure.tex <==
\begin{tikzpicture}

  \node[obs]                               	(y) {$y_i$};
  \node[latent, left=0.5cm of y] 				(fi) {$f_i$};
  \node[latent, left= 0.5cm of fi]  			(f) {$f$};
  \node[const, left=0.5cm of f]            	(gp) {$\mathcal{GP}$};
  \node[latent, left=0.7cm of gp]				(s) {$\sigma_j$};
  \node[const, below=0.5cm of gp]				(kj) {$k_{d_j}(x,x')$};
  \node[const, above=0.6cm of gp]				(ks) {$k_S(x,x')$};
  \node[const, left=0.5cm of ks]				(mu) {$\mu(x)$};
  \node[const, above=0.6cm of mu]				(zero) {$0$};
  \node[latent, right=0.4cm of zero]				(k_s) {$k_S$};
  \node[latent, right =1.6cm of zero]				(theta) {$\theta$};
   \node[const, above=0.5cm of k_s]				(g) {$G$};

%   \node[const, above= of gp, xshift=1.2cm]	(mu) {$\mu(x)$};

  \edge {fi} {y} ;
  \edge {f} {fi} ;
  \edge {gp} {f} ;
  \edge {kj} {gp};
  \edge {ks} {gp};
  \edge {mu} {gp};
  \edge {zero} {mu};
  \edge {g}{k_s};
  \edge {k_s}{ks};
  \edge {theta}{ks};

%   \edge {mu} {gp};
  \edge {s} {gp};

  % Plates
  \plate {fiyi} {(y) (fi)} {$i \in 1 ... N$};
  \plate {M} {(fiyi) (f) (gp) (kj) (s)} {$j \in 1 ... M$}


\end{tikzpicture}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}
